BanglaBERT: Language Model Pretraining and Benchmarks for Low-Resource Language Understanding Evaluation in Bangla

In this work, we introduce BanglaBERT, a BERT-based Natural Language Understanding (NLU) model pretrained in Bangla, a widely spoken yet low-resource language in the NLP literature. To pretrain BanglaBERT, we collect 27.5 GB of Bangla pretraining data (dubbed `Bangla2B+') by crawling 110 popular Bangla sites. We introduce two downstream task datasets on natural language inference and question answering and benchmark on four diverse NLU tasks covering text classification, sequence labeling, and span prediction. In the process, we bring them under the first-ever Bangla Language Understanding Benchmark (BLUB). BanglaBERT achieves state-of-the-art results outperforming multilingual and monolingual models. We are making the models, datasets, and a leaderboard publicly available at https://github.com/csebuetnlp/banglabert to advance Bangla NLP.

==> 5_analysis.tex <==
%\vspace{-6mm}
\section{Analysis \& Discussions}



%In addition to data, we opine the insufficiency of Bangla tokens in the combined vocabulary of mBERT and XLM-R was also a reason behind their under-performance.  \citet{rust-etal-2021-good} showed that languages adequately represented in multilingual models' vocabulary exhibit negligible performance loss over their monolingual counterparts. Having a unique writing script, Bangla has only 2.5k (0.67k) native tokens in XLM-R's (mBERT's) vocabulary, which we hypothesize is too low to convey its morphological richness. Despite being a 270M (180M) parameter base model, being unable to use 70\% (50\%) of the total parameters that are located in the embedding layer, XLM-R (mBERT) faced a barrier in learning representations of Bangla texts.

%placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder text placeholder


==> 8_relworks.tex <==
\section{Related Works}\label{sec:relatedworks}

Natural language processing has witnessed a sea change with the advent of pretrained language models like ULMfit \citep{howard2018universal}, ELMo \citep{peters2018deep}, GPT \citep{radford2019language}, and most notably BERT \citep{devlin-etal-2019-bert}. CamemBERT \citep{martin2019camembert}, trained in French, was one of the first non-English language-specific models. Subsequently, many works \citep{polignano2019alberto, de2019bertje, canete2020spanish, baly2020arabert} did pretraining for other languages.  mBERT \citep{devlin-etal-2019-bert}, XLM \citep{conneau2019cross}, XLM-R \citep{conneau2019unsupervised} explored multilingual pretraining on hundreds of languages and showed cross-lingual effectiveness of multilingual models.

\textbf{Pretraining in Bangla}: Although many Bangla pretrained models (e.g., sahajBERT \citealp{diskin2021distributed}) are publicly available through the Hugging Face Transformers library \citep{wolf2020transformers}, none have pretrained on a high volume of good-quality data (resulting in a sub-par performance, as shown in Table \ref{tab:benchmark}) nor did fine-tune on a variety of tasks.

